Update Frequently, Update Fast: Retraining Semantic Parsing Systems in a Fraction of Time

Currently used semantic parsing systems deployed in voice assistants can require weeks to train. Datasets for these models often receive small and frequent updates, data patches. Each patch requires training a new model. To reduce training time, one can fine-tune the previously trained model on each patch, but naive fine-tuning exhibits catastrophic forgetting - degradation of the model performance on the data not represented in the data patch. In this work, we propose a simple method that alleviates catastrophic forgetting and show that it is possible to match the performance of a model trained from scratch in less than 10% of a time via fine-tuning. The key to achieving this is supersampling and EWC regularization. We demonstrate the effectiveness of our method on multiple splits of the Facebook TOP and SNIPS datasets.

==> 03_methods_v1.tex <==
% We empirically experiment with and explore various fine tuning approaches.

% \textbf{Naive Fine-tuning}: Here we simply take the finetune data and train the network for a fixed number of steps. This typically leads to catastrophic forgeting. 
    
% \textbf{Old data Sampling}: Similar to experience replay in lifelong learning~\citet{de2019episodic}, we sample directly from the pretrain data during finetuning. We study 2 setups: \textit{static sampling} and \textit{dynamic sampling}. 

% \textit{Static sampling} randomly takes a proportion $p where 0 < p \leq 1$ of the pretrain data and mix with the fine-tuning data for the fine tuning procedure. This kind of setup is beneficial for privacy in a federated learning setup where we a limited amount buffer is available during fine-tuning. As this is of the simplest setups to combat catastrophic forgetting we call this \textit{baseline} in our results. 

% \textit{Dynamic sampling} samples the amount of $p$ pretraining data at the beginning of each epoch. In this case, more of the pretrain data gets reused yielding a more diverse dataset, while the epoch length stays the same compared to the static sampling.

% \textbf{Regularization methods}: As the fine-tuning set is usuallay small and its  class distribution is different from the pretraining set, overfitting is expected. Dropout is a standard deep learning tool that helps to deal with this problem. 
%     %TODO(vlad): Say what we do wrt to dropout in our experiments. 

% Elastic Weight Consolidation (EWC)~\cite{Kirkpatrick2017} is the most popular regularization technique to prevent catastrophic forgetting, we experiment with effectiveness of EWC for our setting. Please note that EWC increases the number of parameters stored by the network by three times which might be too costly in some production settings. 
    
% To combat the network size increase during training due to EWC, we introduce a simple method with a single regularization parameter called \textit{move norm}. Similar to EWC,  \textit{move norm} is a regularizer that prevents the model diverging from the pre-trained weights. It is added to the loss function like weight decay and is parametrized by $\lambda$.
% $$R(\Theta, \Theta_{pre-trained}) = \lambda || \Theta - \Theta_{pre-trained}) ||_2 $$
% For the distance between $\Theta$ and $\Theta_{pre-trained}$, we experimented with both
% euclidean (L2) and manhattan (L1) distances and found euclidean to be more effective.

% \textbf{A note on other methods tried which didnt wor} Layer Freezing: This is a popular method to limit how much the fine-tuned model diverges from the pre-trained model. \citet{Howard2018} showed that freezing can reduce test error by about 10\% (relative change).
% Freezing can also be looked at as a ``hard'' form of the move norm regularization. In our freezing experiments we freeze the encoder for the whole fine-tuning procedure.
% % TODO{vlad}: add averaging as another method. 

% % \subsection{Old data sampling}

% % \citet{de2019episodic} proposed to use sparse experience replay to mitigate
% % catastrophic forgetting in lifelong language learning.
% % We follow their idea, but instead of implementing an experience replay, we sample
% % directly from the pretrain data during fine-tuning.

% % We study two setups: static and dynamic sampling.
% % Each of them has its pros and cons.

% % Static sampling takes a proportion of size $0 < p \leq 1$ of the pretrain data before
% % the fine-tuning procedure.
% % Then, the fine-tuning happens on a combined dataset of sampled data and the fine-tune subset,
% % i.e., on the $D_2 \cup S_p(D_1)$ where $S_p$ is a random sampler with probability $p$.
% % In this case, the fine-tuning method only uses a limited amount of pretrain data.
% % This may be beneficial in terms of privacy and in the federated training setup.
% % We would like to note that this method is equivalent to having an experience replay of the size $s = \# pretrain \cdot p$ and sample probability~$\# s / (s + \#fine-tune)$.
% % As this kind of sampling can be considered the simplest way to avoid catastrophic
% % forgetting, we call it \textit{baseline} in our plots.

% % Dynamic sampling samples the amount of $p$ pretraining data at the beginning of each epoch.
% % In this case, more of the data gets reused yielding a more diverse dataset,
% % while the epoch length stays the same compared to the static sampling.
% % This method is equivalent to undersampling the pretrain dataset with parameter $p$.

% % \subsection{Regularization methods}

% % As the fine-tuning set is relatively small and its class distribution is very different
% % from the pretraining set, it is natural to expect overfitting and poor generalization
% % performance. Dropout is a standard deep learning tool that helps
% % to deal with this problem.

% % % and weight decay are

% % We also introduce a simple regularization method similar to weight decay but targeted
% % specifically for Incremental training / Continual learning.
% % Move norm is a regularizer that prevents the model diverging from the pre-trained weights
% % (Equation \ref{eq:move}).
% % It is added to the loss function analogous to weight decay and is parametrized by
% % $\lambda$.

% % \begin{equation}
% %     R(\Theta, \Theta_{pre-trained}) = \lambda || \Theta - \Theta_{pre-trained}) ||_2
% % \label{eq:move}
% % \end{equation}

% % For the distance between $\Theta$ and $\Theta_{pre-trained}$, we experimented with both
% % euclidean (L2) and manhattan (L1) distances and found euclidean to be more effective.

% % \subsection{Layer Freezing}

% % One of the methods to limit how much the fine-tuned model diverges from the pre-trained
% % one is layer freezing - not updating the weights in chosen layers.
% % \citet{Howard2018} showed that freezing can reduce test error by about 10\% (relative change).
% % Freezing can also be looked at as a ``hard'' form of the move norm regularization.


==> 06_results_v1.tex <==
% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=0.47\textwidth]{img/bert_nobert.png}
% %     \caption{BERT encoder (solid line) vs best randomly initialized transformer
% %     (no-BERT, dashed line).}
% %     \label{fig:bert_nobert}
% % \end{figure}

% \begin{figure*}[]
%     \centering
%     \includegraphics[width=0.46\textwidth]{img/path90_f1.png}
%     \includegraphics[width=0.47\textwidth]{img/path90_rd.png}
%     \caption{
%     PATH 90 experiments.
%     The model is fine-tuned on 90\% of the examples containing PATH class
%     with different amounts of pretrain data mixed with the fine-tuning data.
%     % It is clear that the pretraining data mixing is essential as the model fine-tuned
%     % without old data, performs significantly worse than the initial model.
%     Legend description:
%     \textit{initial}~--~train on pretrain set;
%     % , containing only 10\% of the examples with PATH class (but also containing all of the other classes).
%     \textit{from scratch}~--~train on all data;
%     \textit{baseline}~--~merge a part of the pretrain set with the fine-tune set;
%     \textit{dynamic sampling}~--~sample a different subset form the pretrain every epoch;
%     \textit{move norm}~--~regularize the distance to the initial model;
%     \textit{freeze encoder}~-~do not update encoder weights.
%     The training time estimates are approximate and slightly depend on early stopping parameter and the fine-tuning method.
%     }
%     \label{fig:path90}
% \end{figure*}


% % We first measured the effect of BERT encoder on task performance.
% % The results are shown in Figure~\ref{fig:bert_nobert}.
% % To have a more fair comparison we performed a hyperparameter search on no-BERT
% % number of layers and hidden sizes.
% % The best no-BERT model had 4 layers, 4 heads, 256 model hidden size and
% % 1024 ffn hidden size.
% % Expectedly, we see better sample efficiency with BERT.
% % Even with 20\% of the
% % original dataset BERT matches the performance of the full no-BERT model.
% % Since BERT could have a profound effect on the final results, we use BERT in all our experiments.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Baselines}

% We start our experiments by establishing two important baselines.
% The first baseline shows if the fine-tuning procedure
% is useful at all - no fine-tuning. It is simply the performance of the model trained on the \textit{pretrain} (old) subset.
% In our figures, we call this baseline \textit{no finetuning}.
% Table \ref{tab:no-finetuning} contains the metrics (on the validation set)
% of this baseline for the models used in our experiments.
% %
% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width=0.47\textwidth]{img/path99_f1.png}
%     \includegraphics[width=0.47\textwidth]{img/path99_rd.png}\\
%     \includegraphics[width=0.47\textwidth]{img/getweather99_f1.png}
%     \includegraphics[width=0.47\textwidth]{img/getweather99_rd.png}
%     \caption{
%     PATH 99 and GETWEATHER~99 experiments.
%     Compared to PATH~90, degradation decreases more significantly,
%     however performance on PATH class increases less significantly
%     when more of the old data is used.
%     The behavior of GETWEATHER~99 is similar to PATH~99.
%     }
%     \label{fig:path99_getweather99}
% \end{figure*}

% \begin{table}[h]
%     \centering
%     \begin{small}
%     \begin{tabular}{c|c|c}
%         Split         & TP-F1         & EM \\\hline
%         PATH 99       & 0.13 $\pm$ 0.01 & 0.801 $\pm$ 0.003 \\\hline
%         PATH 90       & 0.51 $\pm$ 0.02 & 0.815 $\pm$ 0.002 \\\hline
%         NAME EVENT 95 & 0.61 $\pm$ 0.02 & 0.809 $\pm$ 0.002 \\\hline
%         GETWEATHER 90 & 0.93 $\pm$ 0.01 & 0.911 $\pm$ 0.004 \\\hline
%         GETWEATHER 99 & 0.77 $\pm$ 0.01 & 0.892 $\pm$ 0.004 \\\hline
%     \end{tabular}
%     \end{small}
%     \caption{
%     Performance of the pre-trained models.
%     TP-F1 reported for the split class.
%     Mean and standard deviations are estimated via bootstraping.
%     }
%     \label{tab:no-finetuning}
% \end{table}

% The second baseline is an upper bound for the fine-tuning procedure.
% It is also the standard way to incorporate more data into a model -
% to retrain the whole model from scratch on the merged pretrain+fine-tune dataset.
% This baseline yields high final performance and no catastrophic forgetting as
% all of the data is being used, but also the method is inherently
% slow and computationally expensive.
% In the figures, we call this baseline \textit{from scratch}.
% EM values for this baseline can be found in the Table \ref{tab:from_scratch_em}
% and TP-F1 values in the Table \ref{tab:from_scratch_f1}.

% To estimate this important baseline with a high precision we
% trained 5 models with different random seeds.
% The resulting mean and standard deviation were compared with the bootstrapping method.
% Both bootstrapping and training on multiple random seeds provided similar results,
% hence we chose to only use bootstrapping for the fine-tuning experiments to significantly
% reduce computational requirements.


% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c}
%         Dataset & EM         \\\hline
%         TOP     & 0.819 $\pm$ 0.003 \\\hline
%         SNIPS   & 0.949 $\pm$ 0.002 \\\hline
%     \end{tabular}
%     \caption{
%     Exact match for the models trained on the whole dataset.
%     Mean and standard deviation are estimated via training 5 models with different random seeds.
%     }
%     \label{tab:from_scratch_em}
% \end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{c|c|c}
%         Dataset & Class         & TP-F1         \\\hline
%         TOP     & PATH          & 0.66 $\pm$ 0.01 \\\hline
%         TOP     & NAME EVENT 95 & 0.84 $\pm$ 0.01 \\\hline
%         SNIPS   & GETWEATHER 90 & 0.97 $\pm$ 0.01 \\\hline
%     \end{tabular}
%     \caption{
%     Tree-Path F1 score for selected classes for the models trained on the whole dataset.
%     Mean and standard deviation are estimated via training 5 models with different random seeds.
%     }
%     \label{tab:from_scratch_f1}
% \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{TOP dataset results}

% \paragraph{PATH 90 split.}
% Figure \ref{fig:path90} presents the experimental results on the PATH 90 split.
% In this split, the fine-tuning part contains 90\% of the examples with PATH class and
% the left plot shows its TP-F1 score.
% Surprisingly, even this class degrades if the pretraining data is not used along with
% the fine-tuning data
% (notice that all of the plots at old data = 0 are below the \textit{no-finetuning} baseline).
% There is a 3.5\% relative degradation at this point (old data = 0).
% However, starting from 5\% of pretraining data, the performance on PATH class
% beats the no-fine-tuning baseline.
% Dynamic sampling method, that selects a new subset of the pretraining data every
% epoch is able to reach the performance of the model trained from scratch in $\sim$10
% minutes which is about 10\% of
% the training from scratch time (training from scratch takes 1.5 hours).

% The exact match metric is different from the TP-F1 and RD as
% it is computed on all classes. We can see that model significantly improves when RD is low and TP-F1 is high, as expected (EM plots are available in the Appendix \ref{apx:results}).


% \paragraph{PATH 99 split.}
% This split is more extreme compared to PATH 90.
% The fine-tuning subset contains 99\% of the PATH data and the pretraining
% subset contains only 15 PATH examples (Table \ref{tab:splits}).
% Our experiments (Figure \ref{fig:path99_getweather99}) show that this case benefits faster
% (in terms of the amount of old data needed to overcome no-finetuning baseline)
% and significantly from fine-tuning.
% However, 50\% of the data is needed to reach retraining from scratch performance (Figure \ref{fig:path99_getweather99}).

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{SNIPS dataset results}

% \paragraph{GETWEATHER 99 split.}
% Along with the TOP dataset we also experimented with SNIPS.
% Figure \ref{fig:path99_getweather99} presents the experimental results for this split.
% One extra experiment that we tried with this split is to freeze both encoder and decoder.
% In this setup, we only updated the weights of output projection and pointer network.
% The results show that this method performs substantially worse than the others.
% It may happen because the features the model has learned on the pretrain subset
% are insufficient to correctly classify examples from the new data.
% Thus, the model needs to change its representations to and not only to reweight the existing ones.
% Another reason that can contribute to this behavior is a distribution shift
% between pretrain and fine-tune set,
% as the logit network mainly learns the simplest features such as class frequency.


% More experimental data can be found in the Appendix \ref{apx:results}.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Parametric regularization methods}

% In our experiments, we tried multiple methods to further mitigate catastrophic
% forgetting and overfitting.
% While some of the methods are non-parametric, others, like dropout or move norm
% require parameter tuning.
% To study parameter dependence we selected the most challenging split - NAME EVENT 95,
% and fine-tuned multiple models with different regularization parameter values.

% % \paragraph{Dropout.}
% % Dropout has become a default regularization choice in modern NLP.
% \textbf{Dropout:} Our initial results showed that the model easily fits the whole fine-tuning
% set and we decided that a slight increase in dropout probability may be beneficial
% \footnote{We used 0.2 dropout during pretraining.}. Nonetheless, our results (Figure \ref{fig:move_norm_dropout}) suggest
% that increasing dropout does not improve fine-tuning performance and that large dropout
% probabilities can significantly hurt underrepresented in the fine-tuning data classes.

% % TODO: recompute L2 with dropout=0.2
% % \paragraph{Weight decay.}
% % Another standard method of regularization is weight decay.
% % To test it, we used dropout=0

% %\paragraph{Move norm.}
% \textbf{Move norm:} This method, unlike dropout, is specifically targeted to mitigate catastrophic forgetting.
% However, unlike the freezing or sampling methods,
% it requires careful parameter tuning as we
% demonstrate in Figure \ref{fig:move_norm_dropout}.
% While the move norm did not improve the results significantly in the NAME EVENT 95 split,
% we can see positive examples in PATH~99~(Figure~\ref{fig:path99_getweather99}).
% Another advantage of move-norm is that the high regularization strengths
% do not cause the model to degrade its
% performance on the classes underrepresented in the fine-tuning data.

% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.47\textwidth]{img/name_event95_dropout.png}
%     \includegraphics[width=0.47\textwidth]{img/name_event95_dropout_rd.png}\\
%     \includegraphics[width=0.47\textwidth]{img/name_event95_move.png}
%     \includegraphics[width=0.47\textwidth]{img/name_event95_move_rd.png}
%     \caption{
%     Dropout probability and move norm regularization strength variation experiments.
%     NAME EVENT 95 split.
%     The high move norm, unlike dropout, does not increase RD.
%     }
%     \label{fig:move_norm_dropout}
% \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Practical Recommendations
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

